Transferring Semantic Roles Using Translation and Syntactic Information

Our paper addresses the problem of annotation projection for semantic role labeling for resource-poor languages using supervised annotations from a resource-rich language through parallel data. We propose a transfer method that employs information from source and target syntactic dependencies as well as word alignment density to improve the quality of an iterative bootstrapping method. Our experiments yield a $3.5$ absolute labeled F-score improvement over a standard annotation projection method.

==> bootstrap.tex <==
\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LState{\State \algbackskip}%
\makeatother

\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LComment{\Comment \algbackskip}%
\makeatother

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{figure}[t!]
\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.2cm}
%\noindent\rule{0.5\textwidth}{0.4pt}
\begin{algorithmic}[0]
\small
 \LState {{\bf Inputs: }{1) Projected data ${\cal D}= {\cal D^L} \cup {\cal D^U}$} where ${\cal D^L}$ and ${\cal D^U}$ indicate labeled and unlabeled instances in the projected data; 2) Number of self-training iterations {\bf $m$}. } 
\vspace{0.2cm}
\LState{\bf Algorithm:}
\State Train model $\theta^0$ on ${\cal D^L}$
\For {$i$ = 1 to $m$}

\State ${\cal D^U}\leftarrow$ Label data ${\cal D^U}$ with model $\theta^{i-1}$.
\State ${\cal D^L}\leftarrow$  Relabel data ${\cal D^L}$ with model $\theta^{i-1}$. 
\State Train model $\theta^{i}$ on ${\cal D^L} \cup {\cal D^U}$
\EndFor

\LState {{\bf Output: } The model parameters $\theta^m$.}
\end{algorithmic}

\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{The iterative bootstrapping algorithm for training SRL on partially projected data.}\label{fig_bootstrap}

\end{figure}

==> data_sizes.tex <==
\begin{table}[t!]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{c c c c  c }
    \hline  \hline
       Sen.  &  Instances & \%Labeled & \%Non-null Args \\
       29417  & 2.1M & 79.8 & 9.7 \\ \hline  \hline
    \end{tabular}
    \caption{Projected data size after filtering sparse alignments.}
    \label{tab_data_size}
\end{table}



==> dep_match_w_srl.tex <==
\begin{figure}
\centering
\begin{subfigure}[t]{0.5\textwidth}

\centering
\begin{dependency}[theme = iron]
\begin{deptext}
I\&would\&urge\&you\&to\&endorse\&this\\
\\
\\
\\
Ich\&bitte\&Sie\&um\&Zustimmung\&\\
\end{deptext}

\depedge{3}{1}{A0}
\depedge{3}{2}{AM-MOD}
\depedge{3}{4}{A1}
\depedge{3}{6}{A2}
\depedge{6}{4}{A0}
\depedge{6}{7}{A1}
													
													
\depedge[dashed,edge below,color=purple]{2}{1}{A0}
\depedge[dashed,edge below,color=purple]{2}{3}{A1}
\depedge[dashed,edge below,color=purple]{2}{5}{A2}
\depedge[dashed,edge below,color=purple]{5}{3}{A0}


\path[dashed,color=blue] (\wordref{1}{1}) edge (\wordref{5}{1});
\path[dashed,color=blue] (\wordref{1}{3}) edge (\wordref{5}{2});
\path[dashed,color=blue] (\wordref{1}{4}) edge (\wordref{5}{3});
\path[dashed,color=blue] (\wordref{1}{6}) edge (\wordref{5}{5});

\wordgroup[color=purple]{1}{3}{3}{pred}
\wordgroup[color=blue]{1}{6}{6}{pred}

\wordgroup[color=purple]{5}{2}{2}{pred}
\wordgroup[color=blue]{5}{5}{5}{pred}

\end{dependency}
\caption{}
\label{error_anal_example_a}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.5\textwidth}
\centering
\begin{dependency}[theme = iron]
\begin{deptext}
Ich\&bitte\&Sie\&um\&Zustimmung\&\\
\end{deptext}
													
\depedge{2}{1}{A0}
\depedge{2}{3}{A1}
%\depedge{2}{5}{A2}
\depedge{5}{3}{A0}


\end{dependency}
\caption{}
\label{fig:dep_match_w_srl}
\end{subfigure}

\caption{(a) Transferring semantic roles for the English-German sentences demonstrated in Figure~\ref{error_anal_example2} using intersected word alignments (shown with dashed lines) from GIZA++ (b) German semantic role labels after the first iteration of relabeling.}
\end{figure}

==> tab_sparsity.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l |c }
    \hline \hline
    Density\% & SRL match \\ \hline  
        $d \leq40\%$ &  \\
         $40\%< d\leq 60\%$&  \\
         $60\%< d\leq 80\%$&  \\
          $d >80\%$ &  \\ \hline \hline
    \end{tabular}
    \caption{The SRL match between the supervised and projected label in the German Europarl data on different alignment density level.}
    \label{tab_sparse}
\end{table}
